On the Exact Amount of Missing Information that makes Finding Possible Winners Hard

We consider election scenarios with incomplete information, a situation that arises often in practice. There are several models of incomplete information and accordingly, different notions of outcomes of such elections. In one well-studied model of incompleteness, the votes are given by partial orders over the candidates. In this context we can frame the problem of finding a possible winner, which involves determining whether a given candidate wins in at least one completion of a given set of partial votes for a specific voting rule. The possible winner problem is well-known to be NP-complete in general, and it is in fact known to be NP-complete for several voting rules where the number of undetermined pairs in every vote is bounded only by some constant. In this paper, we address the question of determining precisely the smallest number of undetermined pairs for which the possible winner problem remains NP-complete. In particular, we find the exact values of $t$ for which the possible winner problem transitions to being NP-complete from being in P, where $t$ is the maximum number of undetermined pairs in every vote. We demonstrate tight results for a broad subclass of scoring rules which includes all the commonly used scoring rules (such as plurality, veto, Borda, $k$-approval, and so on), Copeland$^\alpha$ for every $\alpha\in[0,1]$, maximin, and Bucklin voting rules. A somewhat surprising aspect of our results is that for many of these rules, the possible winner problem turns out to be hard even if every vote has at most one undetermined pair of candidates.

==> preamble.tex <==
\usepackage{amssymb,amsmath,amsthm}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{thmtools,thm-restate}
\usepackage{datetime}
\usepackage{relsize}
\usepackage{fullpage}
\usepackage[usenames,dvipsnames,svgnames]{xcolor}
\usepackage[colorlinks=true,linkcolor=blue,citecolor=Mahogany]{hyperref}
\sloppy

\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}

\usepackage{url}

\makeatletter
\newcommand{\mathleft}{\@fleqntrue\@mathmargin\parindent}
\newcommand{\mathcenter}{\@fleqnfalse}
\makeatother

\usepackage{xspace}

\newcommand{\el}{\ensuremath{\ell}\xspace}
\newcommand{\suc}{\ensuremath{\succ}\xspace}

\renewcommand{\labelitemi}{--}

\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\argmax}{arg\!max}

\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\YES}{\textsc{Yes}\xspace}
\newcommand{\NO}{\textsc{No}\xspace}

\newcommand{\BigO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\true}{\textsc{true}\xspace}
\newcommand{\false}{\textsc{false}\xspace}
\newcommand{\pr}{\ensuremath{\prime}\xspace}
\newcommand{\prr}{{\ensuremath{\prime\prime}}\xspace}
\newcommand{\prm}{{\ensuremath{\prime}}\xspace}
\newcommand{\PE}{\textsc{Preference Elicitation}\xspace}
\newcommand{\CW}{\textsc{Weak Condorcet Winner}\xspace}
\newcommand{\WCW}{\textsc{Weak Condorcet Winner}\xspace}
\newcommand{\WD}{\textsc{Winner Determination}\xspace}
\newcommand{\WM}{\ensuremath{\mathsf{WM}}\xspace}
\newcommand{\SM}{\ensuremath{\mathsf{SM}}\xspace}
\newcommand{\OM}{\ensuremath{\mathsf{OM}}\xspace}
\newcommand{\CM}{\ensuremath{\mathsf{CM}}\xspace}
\newcommand{\PW}{\textsc{Possible Winner}\xspace}
\newcommand{\TDM}{\textsc{Three Dimensional Matching}\xspace}
\newcommand{\MIS}{\textsc{Multicolored Independent Set}\xspace}
\newcommand{\VC}{\textsc{Vertex Cover}\xspace}
\newcommand{\NW}{\ensuremath{\mathsf{NW}}\xspace}
\newcommand{\SAT}{\ensuremath{(3,B2)}--\textsc{SAT}\xspace}

\newcommand{\NP}{\ensuremath{\mathsf{NP}}\xspace}
\newcommand{\Pb}{\ensuremath{\mathsf{P}}\xspace}
\newcommand{\coNP}{\ensuremath{\mathsf{co}}-\ensuremath{\mathsf{NP}}\xspace}
\newcommand{\coNPH}{\ensuremath{\mathsf{co}}-\ensuremath{\mathsf{NP}}-hard\xspace}
\newcommand{\NPH}{\ensuremath{\mathsf{NP}}-hard\xspace}
\newcommand{\NPC}{\ensuremath{\mathsf{NP}}-complete\xspace}

\newcommand{\caveat}{\ensuremath{\mathsf{CoNP\subseteq NP/Poly}}\xspace}

\newcommand{\RB}{\ensuremath{\mathbb R}\xspace}
\newcommand{\SB}{\ensuremath{\mathbb S}\xspace}
\newcommand{\NB}{\ensuremath{\mathbb N}\xspace}
\newcommand{\PB}{\ensuremath{\mathbb P}\xspace}
\newcommand{\EB}{\ensuremath{\mathbb E}\xspace}

\newcommand{\SF}{\ensuremath{\mathfrak S}\xspace}
\newcommand{\PF}{\ensuremath{\mathfrak P}\xspace}

\renewcommand{\AA}{\ensuremath{\mathcal A}\xspace}
\newcommand{\BB}{\ensuremath{\mathcal B}\xspace}
\newcommand{\CC}{\ensuremath{\mathcal C}\xspace}
\newcommand{\DD}{\ensuremath{\mathcal D}\xspace}
\newcommand{\EE}{\ensuremath{\mathcal E}\xspace}
\newcommand{\FF}{\ensuremath{\mathcal F}\xspace}
\newcommand{\GG}{\ensuremath{\mathcal G}\xspace}
\newcommand{\HH}{\ensuremath{\mathcal H}\xspace}
\newcommand{\II}{\ensuremath{\mathcal I}\xspace}
\newcommand{\JJ}{\ensuremath{\mathcal J}\xspace}
\newcommand{\KK}{\ensuremath{\mathcal K}\xspace}
\newcommand{\LL}{\ensuremath{\mathcal L}\xspace}
\newcommand{\MM}{\ensuremath{\mathcal M}\xspace}
\newcommand{\NN}{\ensuremath{\mathcal N}\xspace}
\newcommand{\OO}{\ensuremath{\mathcal O}\xspace}
\newcommand{\PP}{\ensuremath{\mathcal P}\xspace}
\newcommand{\QQ}{\ensuremath{\mathcal Q}\xspace}
\newcommand{\RR}{\ensuremath{\mathcal R}\xspace}
\renewcommand{\SS}{\ensuremath{\mathcal S}\xspace}
\newcommand{\TT}{\ensuremath{\mathcal T}\xspace}
\newcommand{\UU}{\ensuremath{\mathcal U}\xspace}
\newcommand{\VV}{\ensuremath{\mathcal V}\xspace}
\newcommand{\WW}{\ensuremath{\mathcal W}\xspace}
\newcommand{\XX}{\ensuremath{\mathcal X}\xspace}
\newcommand{\YY}{\ensuremath{\mathcal Y}\xspace}
\newcommand{\ZZ}{\ensuremath{\mathcal Z}\xspace}

\newcommand{\aaa}{\ensuremath{\mathfrak a}\xspace}
\newcommand{\bbb}{\ensuremath{\mathfrak b}\xspace}
\newcommand{\ccc}{\ensuremath{\mathfrak c}\xspace}
\newcommand{\ddd}{\ensuremath{\mathfrak d}\xspace}
\newcommand{\eee}{\ensuremath{\mathfrak e}\xspace}
\newcommand{\fff}{\ensuremath{\mathfrak f}\xspace}
\renewcommand{\ggg}{\ensuremath{\mathfrak g}\xspace}
\newcommand{\hhh}{\ensuremath{\mathfrak h}\xspace}
\newcommand{\iii}{\ensuremath{\mathfrak i}\xspace}
\newcommand{\jjj}{\ensuremath{\mathfrak j}\xspace}
\newcommand{\kkk}{\ensuremath{\mathfrak k}\xspace}
\renewcommand{\lll}{\ensuremath{\mathfrak l}\xspace}
\newcommand{\mmm}{\ensuremath{\mathfrak m}\xspace}
\newcommand{\nnn}{\ensuremath{\mathfrak n}\xspace}
\newcommand{\ooo}{\ensuremath{\mathfrak o}\xspace}
\newcommand{\ppp}{\ensuremath{\mathfrak p}\xspace}
\newcommand{\qqq}{\ensuremath{\mathfrak q}\xspace}
\newcommand{\rrr}{\ensuremath{\mathfrak r}\xspace}
\newcommand{\sss}{\ensuremath{\mathfrak s}\xspace}
\newcommand{\ttt}{\ensuremath{\mathfrak t}\xspace}
\newcommand{\uuu}{\ensuremath{\mathfrak u}\xspace}
\newcommand{\vvv}{\ensuremath{\mathfrak v}\xspace}
\newcommand{\www}{\ensuremath{\mathfrak w}\xspace}
\newcommand{\xxx}{\ensuremath{\mathfrak x}\xspace}
\newcommand{\yyy}{\ensuremath{\mathfrak y}\xspace}
\newcommand{\zzz}{\ensuremath{\mathfrak z}\xspace}

\newcommand{\bCC}{\overline{\mathcal{C}}\xspace}


\usepackage{nicefrac}
\newcommand{\ffrac}{\flatfrac}
\newcommand{\nfrac}{\nicefrac}

\newcommand{\defparproblem}[4]{
  \vspace{1mm}
\begin{center}
\noindent\fbox{

  \begin{minipage}{\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1}  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
 
  }
\end{center}
  \vspace{1mm}
}

\newtheorem{proposition}{\bf Proposition}
\newtheorem{observation}{\bf Observation}
\newtheorem{theorem}{\bf Theorem}
\newtheorem{lemma}{\bf Lemma}
\newtheorem{claim}{\bf Claim}
\newtheorem{corollary}{\bf Corollary}
\newtheorem{definition}{\bf Definition}
\newtheorem{reductionrule}{\bf Reduction rule}

\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\eps}

\usepackage{charter}

%Clever References
\usepackage{cleveref}

\crefname{theorem}{theorem}{\bf Theorem}
\crefname{observation}{observation}{\bf Observation}
\crefname{lemma}{lemma}{\bf Lemma}
\crefname{corollary}{corollary}{\bf Corollary}
\crefname{proposition}{proposition}{\bf Proposition}
\crefname{definition}{definition}{\bf Definition}
\crefname{claim}{claim}{\bf Claim}
\crefname{reductionrule}{reduction rule}{\bf Reduction rule}
\crefname{chapter}{chapter}{\bf Chapter}



\newcommand{\nice}{smooth}
\usepackage[obeyDraft]{todonotes}
\newcommand{\addref}{\todo[color=MistyRose]{Ref!}}

% Author specific comment commands

\newcounter{nmcomment}
\newcommand{\nmtodo}[1]{%
    % initials of the author (optional) + note in the margin
    \refstepcounter{nmcomment}%
    {%
        \todo[color={LightSteelBlue},size=\small,inline]{%
            \textbf{Comment [NM\thenmcomment ]:}~#1}%
}}


\newcounter{pdcomment}
\newcommand{\pdtodo}[1]{%
    % initials of the author (optional) + note in the margin
    \refstepcounter{pdcomment}%
    {%
        \todo[color={LightCoral},size=\small,inline]{%
            \textbf{Comment [pd\thepdcomment ]:}~#1}%
}}


